Hierarchical Contrastive Learning for Pattern-Generalizable Image Corruption Detection

Effective image restoration with large-size corruptions, such as blind image inpainting, entails precise detection of corruption region masks which remains extremely challenging due to diverse shapes and patterns of corruptions. In this work, we present a novel method for automatic corruption detection, which allows for blind corruption restoration without known corruption masks. Specifically, we develop a hierarchical contrastive learning framework to detect corrupted regions by capturing the intrinsic semantic distinctions between corrupted and uncorrupted regions. In particular, our model detects the corrupted mask in a coarse-to-fine manner by first predicting a coarse mask by contrastive learning in low-resolution feature space and then refines the uncertain area of the mask by high-resolution contrastive learning. A specialized hierarchical interaction mechanism is designed to facilitate the knowledge propagation of contrastive learning in different scales, boosting the modeling performance substantially. The detected multi-scale corruption masks are then leveraged to guide the corruption restoration. Detecting corrupted regions by learning the contrastive distinctions rather than the semantic patterns of corruptions, our model has well generalization ability across different corruption patterns. Extensive experiments demonstrate following merits of our model: 1) the superior performance over other methods on both corruption detection and various image restoration tasks including blind inpainting and watermark removal, and 2) strong generalization across different corruption patterns such as graffiti, random noise or other image content. Codes and trained weights are available at https://github.com/xyfJASON/HCL .

==> tables/table1.tex <==
\begin{table}[!t]
\centering
\caption{Performance comparison for mask detection on three benchmark datasets for blind image inpainting.
%the FFHQ~\cite{karras2019style}, ImageNet~\cite{deng2009imagenet}, and Places~\cite{zhou2017places} datasets. %Metrics with $\uparrow$, higher value denotes better performance, whereas $\downarrow$ denotes lower is better. 
%The best results of each metric are highlighted in \textbf{bold}.
}
%\renewcommand\arraystretch{1.2}
\resizebox{0.8\linewidth}{!}{
\begin{tabular}{c |l| c c c c c c}
\toprule
%\multirow{2}*{Metric}&\multirow{2}*{Method}
\multicolumn{2}{c|}{Dataset}&\multicolumn{2}{c}{FFHQ~\cite{karras2019style}} &\multicolumn{2}{c}{ImageNet~\cite{deng2009imagenet}}&\multicolumn{2}{c}{Places~\cite{zhou2017places}} \\
% \cmidrule(lr){3-5} 
% \cmidrule(lr){6-8}
% \cmidrule(lr){9-11}
\cmidrule(lr){1-2}
\cmidrule(lr){3-4} 
\cmidrule(lr){5-6}
\cmidrule(lr){7-8}
%~&&small&large&small&large&small&large\\
\multicolumn{2}{c|}{Mask ratio (\%)}&0-30&30-60&0-30&30-60&0-30&30-60\\
\midrule
\multirow{2}*{Acc~$\uparrow$}&VCNet&0.948&0.943&0.972&0.978&0.974&0.976 \\
~&Ours&\textbf{0.978}&\textbf{0.976}&\textbf{0.982}&\textbf{0.983}&\textbf{0.984}&\textbf{0.985} \\
\midrule
\multirow{2}*{F1~$\uparrow$}&VCNet&0.967&0.948&0.982&0.980&0.984&0.978\\
~&Ours&\textbf{0.986}&\textbf{0.978}&\textbf{0.989}&\textbf{0.985}&\textbf{0.991}&\textbf{0.987} \\
\midrule
\multirow{2}*{BCE~$\downarrow$}&VCNet&0.126&0.137&\textbf{0.073}&\textbf{0.055}&\textbf{0.064}&\textbf{0.060} \\
~&Ours&\textbf{0.090}&\textbf{0.095}&0.083&0.075&0.068&0.064 \\
\midrule
\multirow{2}*{IoU~$\uparrow$}&VCNet&0.931&0.900&0.966&0.962&0.969&0.959 \\
~&Ours&\textbf{0.975}&\textbf{0.959}&\textbf{0.978}&\textbf{0.965}&\textbf{0.982}&\textbf{0.974} \\
\bottomrule
\end{tabular}}
\label{tab1:mask}
\vspace{-4pt}
\end{table} 

\begin{comment}
% here is a larger table
\end{comment}

==> tables/table11.tex <==
%\vspace{-6pt}
\begin{table}[!t]
\centering
\caption{Computational overhead.}
\vspace{-10pt}
%\renewcommand\arraystretch{1.2}
\resizebox{0.95\linewidth}{!}{
\begin{tabular}{l | cccc}
\toprule
Metrics&Params (M)&Memory usage (GB)&MACs&Inference time (ms) \\
\midrule
VCNet      &3.88          &1.65  &$3.1\times10^9$ &15.3 \\
Our model  &3.57 &1.97           &$3.7\times10^9$ &29.1 (28.7 for Transformer) \\
\bottomrule
\end{tabular}
 }
\label{tab7:overhead}
%\vspace{-12pt}
\end{table} 


==> tables/table12.tex <==
%\vspace{-13pt}
\begin{table}[!t]
\centering
\caption{Performance evaluation on bidirectional blind image inpainting.}
%\vspace{-8pt}
%\renewcommand\arraystretch{1.2}
\resizebox{1\linewidth}{!}{
\begin{tabular}{l | ccc | ccc| ccc| ccc}
\toprule
Metrics&\multicolumn{3}{c|}{Acc~$\uparrow$}&\multicolumn{3}{c|}{F1~$\uparrow$}&\multicolumn{3}{c|}{BCE~$\downarrow$}&\multicolumn{3}{c}{IoU~$\uparrow$} \\
\cmidrule(lr){0-1} 
\cmidrule(lr){2-4} 
\cmidrule(lr){5-7} 
\cmidrule(lr){8-10}
\cmidrule(lr){11-13}
Mask ratio (\%)&0-20&20-40&40-60 &0-20&20-40&40-60 &0-20&20-40&40-60 &0-20&20-40&40-60  \\
\midrule
VCNet &0.899&0.826&0.760&0.938&0.866&0.770&0.228&0.378&0.569&0.887&0.772&0.645 \\
Our model  &\textbf{0.978}&\textbf{0.968}&\textbf{0.973}&\textbf{0.987}& \textbf{0.979}    &\textbf{0.973}&\textbf{0.084}&\textbf{0.124}&\textbf{0.105}&\textbf{0.975}&\textbf{0.955}&\textbf{0.947} \\
\bottomrule
\end{tabular}
 }
\label{tab4:mask}
\end{table} 
%\vspace{-10pt}

==> tables/table2.tex <==
%\begin{comment}
% here is a larger table
\begin{table*}[!t]
\centering
\caption{Performance comparison for blind image inpainting in terms of four evaluation metrics on three benchmark datasets.
%the FFHQ~\cite{karras2019style}, ImageNet~\cite{deng2009imagenet}, and Places2~\cite{zhou2017places} datasets.
}
%\renewcommand\arraystretch{1.2}
\resizebox{0.6\linewidth}{!}{
\begin{tabular}{c| l| c c c c| c c c c| c c c c}
\toprule
\multicolumn{2}{c|}{Dataset}&\multicolumn{4}{c|}{FFHQ~\cite{karras2019style}} &\multicolumn{4}{c|}{ImageNet~\cite{deng2009imagenet}}&\multicolumn{4}{c}{Places~\cite{zhou2017places}} \\
\cmidrule(lr){1-2} 
\cmidrule(lr){3-6} 
\cmidrule(lr){7-10}
\cmidrule(lr){11-14}
\multicolumn{2}{c|}{Mask ratio (\%)}&0-20 & 20-40 & 40-60 & 0-60 &0-20 & 20-40 & 40-60 & 0-60 &0-20 & 20-40 & 40-60 & 0-60 \\
\midrule
\multirow{2}*{PSNR~$\uparrow$}&VCNet&29.86&24.51&20.51&24.96&29.13&23.39&19.42&23.98&29.66&23.19&19.18&24.01 \\
~&Ours&\textbf{34.79}&\textbf{27.98}&\textbf{23.54}&\textbf{28.77}&\textbf{33.91}&\textbf{26.40}&\textbf{21.80}&\textbf{27.37}&\textbf{34.11}&\textbf{26.20}&\textbf{21.66}&\textbf{27.32} \\
\midrule
\multirow{2}*{SSIM~$\uparrow$}&VCNet&0.933&0.849&0.736&0.839&0.924&0.818&0.678&0.807&0.942&0.833&0.688&0.821 \\
~&Ours&\textbf{0.971}&\textbf{0.910}&\textbf{0.824}&\textbf{0.901}&\textbf{0.966}&\textbf{0.884}&\textbf{0.767}&\textbf{0.872}&\textbf{0.969}&\textbf{0.887}&\textbf{0.746}&\textbf{0.873} \\
\midrule
\multirow{2}*{FID~$\downarrow$}&VCNet&6.80&14.17&28.90&16.63&5.69&21.48&59.11&28.76&5.93&18.62&40.21&21.59 \\
~&Ours&\textbf{2.37}&\textbf{7.28}&\textbf{15.48}&\textbf{8.38}&\textbf{2.69}&\textbf{12.35}&\textbf{41.37}&\textbf{18.80}&\textbf{2.88}&\textbf{11.10}&\textbf{31.33}&\textbf{15.10} \\
\midrule
\multirow{2}*{LPIPS~$\downarrow$}&VCNet&0.044&0.103&0.188&0.112&0.045&0.128&0.246&0.140&0.046&0.138&0.261&0.148 \\
~&Ours&\textbf{0.019}&\textbf{0.065}&\textbf{0.139}&\textbf{0.075}&\textbf{0.025}&\textbf{0.098}&\textbf{0.226}&\textbf{0.116}&\textbf{0.024}&\textbf{0.095}&\textbf{0.221}&\textbf{0.113} \\
\bottomrule
\end{tabular}
 }
\label{tab2:blind}
\end{table*} 
%\end{comment}







\begin{comment}
% here is a small table
\begin{table}[!t]
\centering
\caption{Performance comparison for blind image inpainting in terms of PSNR and SSIM on the FFHQ~\cite{}, ImageNet~\cite{}, and Places~\cite{} datasets.}
%\renewcommand\arraystretch{1.2}
\resizebox{1\linewidth}{!}{
\begin{tabular}{c |l| c c c c c c}
\toprule
\multicolumn{2}{c|}{Dataset}&\multicolumn{2}{c}{FFHQ} &\multicolumn{2}{c}{ImageNet}&\multicolumn{2}{c}{Places} \\
\cmidrule(lr){1-2}
\cmidrule(lr){3-4} 
\cmidrule(lr){5-6}
\cmidrule(lr){7-8}
\multicolumn{2}{c|}{Mask ratio (\%)}&0-30&30-60&0-30&30-60&0-30&30-60\\
\midrule
\multirow{2}*{PSNR~$\uparrow$}&VCNet&&&&&& \\
~&Ours&&&&&& \\
\midrule
\multirow{2}*{SSIM~$\uparrow$}&VCNet&&&&&&\\
~&Ours&&&&&& \\
\midrule
\multirow{2}*{LPIPS~$\downarrow$}&VCNet&&&&&& \\
~&Ours&&&&&& \\
\bottomrule
\end{tabular}}
\label{tab:center}
\vspace{-4pt}
\end{table} 
\end{comment}


==> tables/table3.tex <==
\begin{table}[!t]
\centering
\caption{\fengx{Ablation study on hierarchical interaction mechanism.}}
%\renewcommand\arraystretch{1.2}
\resizebox{0.8\linewidth}{!}{
\begin{tabular}{c |l| c c c c}
\toprule
%\multirow{2}*{Metric}&\multirow{2}*{Method}
\multicolumn{2}{c|}{Dataset}&\multicolumn{2}{c}{FFHQ} &\multicolumn{2}{c}{Places} \\
% \cmidrule(lr){3-5} 
% \cmidrule(lr){6-8}
% \cmidrule(lr){9-11}
\cmidrule(lr){1-2}
\cmidrule(lr){3-4} 
\cmidrule(lr){5-6}
%~&&small&large&small&large&small&large\\
\multicolumn{2}{c|}{Mask ratio (\%)}&0-30&30-60&0-30&30-60\\
\midrule
\multirow{3}*{Acc~$\uparrow$}&w/o inter-stage consistency&0.969&0.965&0.979&0.978 \\
~&w/o sample selection&0.976&0.975&0.982&0.984 \\
~&Complete model&\textbf{0.978}&\textbf{0.976}&\textbf{0.984}&\textbf{0.985} \\
\midrule
\multirow{3}*{F1~$\uparrow$}&w/o inter-stage consistency&0.980&0.969&0.986&0.980 \\
~&w/o sample selection&0.985&0.977&0.989&0.986 \\
~&Complete model&\textbf{0.986}&\textbf{0.978}&\textbf{0.991}&\textbf{0.987} \\
\midrule
\multirow{3}*{BCE~$\downarrow$}&w/o inter-stage consistency&0.102&0.115&0.089&0.093\\
~&w/o sample selection&0.092&0.096&0.068&0.066 \\
~&Complete model&\textbf{0.090}&\textbf{0.095}&0.068&0.064 \\
\midrule
\multirow{3}*{IoU~$\uparrow$}&w/o inter-stage consistency&0.962&0.940&0.975&0.961\\
~&w/o sample selection&0.973&0.957&0.981&0.972 \\
~&Complete model&\textbf{0.975}&\textbf{0.959}&\textbf{0.982}&\textbf{0.974} \\
\bottomrule
\end{tabular}}
\label{tab3:ablation}
%\vspace{-4pt}
\end{table} 

\begin{comment}
% here is a larger table
\end{comment}

==> tables/table4.tex <==
\begin{table}[!t]
\centering
\caption{Performance comparison of model generalization for mask detection. Both models are first trained on Places dataset~\cite{zhou2017places}.
%Metrics with $\uparrow$, higher value denotes better performance, whereas $\downarrow$ denotes lower is better. 
%The best results of each metric are highlighted in \textbf{bold}.
}
%\renewcommand\arraystretch{1.2}
\resizebox{0.6\linewidth}{!}{
\begin{tabular}{c |l| c c c c}
\toprule
%\multirow{2}*{Metric}&\multirow{2}*{Method}
\multicolumn{2}{c|}{Corruption pattern}&\multicolumn{2}{c}{Random constant}&\multicolumn{2}{c}{CelebA-HQ~\cite{karras2018progressive}} \\
\cmidrule(lr){1-2}
\cmidrule(lr){3-4} 
\cmidrule(lr){5-6}
\multicolumn{2}{c|}{Mask ratio (\%)}&0-30&30-60&0-30&30-60\\
\midrule
\multirow{2}*{Acc~$\uparrow$}&VCNet&0.981&0.977&0.975&0.974 \\
~&Ours&\textbf{0.990}&\textbf{0.989}&\textbf{0.986}&\textbf{0.986} \\
\midrule
\multirow{2}*{F1~$\uparrow$}&VCNet&0.988&0.978&0.984&0.976\\
~&Ours&\textbf{0.994}&\textbf{0.990}&\textbf{0.992}&\textbf{0.988} \\
\midrule
\multirow{2}*{BCE~$\downarrow$}&VCNet&\textbf{0.050}&0.078&0.063&0.068 \\
~&Ours&\textbf{0.050}&\textbf{0.049}&\textbf{0.062}&\textbf{0.054} \\
\midrule
\multirow{2}*{IoU~$\uparrow$}&VCNet&0.977&0.960&0.969&0.954 \\
~&Ours&\textbf{0.988}&\textbf{0.981}&\textbf{0.983}&\textbf{0.976} \\
\bottomrule
\end{tabular}}
\label{tab3:general}
%\vspace{-4pt}
\end{table} 

\begin{comment}
% here is a larger table
\end{comment}

==> tables/table5.tex <==
%\begin{comment}
% here is a larger table
\begin{table}[!t]
\centering
\caption{Performance comparison of model generalization for blind inpainting. Both models are first trained on Places dataset~\cite{zhou2017places}.}
%\renewcommand\arraystretch{1.2}
\resizebox{0.95\linewidth}{!}{
\begin{tabular}{c| l| c c c c| c c c c}
\toprule
\multicolumn{2}{c|}{Corruption Pattern}&\multicolumn{4}{c|}{Random constant} &\multicolumn{4}{c}{CelebA-HQ~\cite{karras2018progressive}} \\
\cmidrule(lr){1-2} 
\cmidrule(lr){3-6} 
\cmidrule(lr){7-10}
\multicolumn{2}{c|}{Mask ratio (\%)}&0-20 & 20-40 & 40-60 & 0-60 &0-20 & 20-40 & 40-60 & 0-60\\
\midrule
\multirow{2}*{PSNR~$\uparrow$}&VCNet&30.48&24.33&19.30&24.70&29.77&23.21&18.96&23.98 \\
~&Ours&\textbf{37.69}&\textbf{29.01}&\textbf{23.05}&\textbf{29.92}&\textbf{34.60}&\textbf{26.52}&\textbf{21.82}&\textbf{27.64} \\
\midrule
\multirow{2}*{SSIM~$\uparrow$}&VCNet&0.957&0.876&0.732&0.855&0.947&0.840&0.685&0.824 \\
~&Ours&\textbf{0.985}&\textbf{0.933}&\textbf{0.818}&\textbf{0.912}&\textbf{0.972}&\textbf{0.894}&\textbf{0.772}&\textbf{0.879} \\
\midrule
\multirow{2}*{FID~$\downarrow$}&VCNet&6.41&16.84&42.54&21.93&5.47&17.75&41.19&21.47\\
~&Ours&\textbf{1.80}&\textbf{7.45}&\textbf{24.48}&\textbf{11.24}&\textbf{2.65}&\textbf{10.50}&\textbf{30.42}&\textbf{14.52}\\
\midrule
\multirow{2}*{LPIPS~$\downarrow$}&VCNet&0.051&0.131&0.268&0.149&0.041&0.128&0.256&0.141 \\
~&Ours&\textbf{0.013}&\textbf{0.063}&\textbf{0.182}&\textbf{0.086}&\textbf{0.021}&\textbf{0.089}&\textbf{0.214}&\textbf{0.108} \\
\bottomrule
\end{tabular}
 }
\label{tab5:general}
\end{table} 
%\end{comment}








==> tables/table6.tex <==
\begin{table}[!t]
\centering
\caption{Experiments on different depths.}
\vspace{-8pt}
%\renewcommand\arraystretch{1.2}
\resizebox{0.5\linewidth}{!}{
\begin{tabular}{c| c| c| c| c}
\toprule
%\multirow{2}*{Metric}&\multirow{2}*{Method}
Depth&1&2&3&4 \\
\midrule
F1~$\uparrow$&0.967&0.984&\textbf{0.986}&0.982 \\
\midrule
IoU~$\uparrow$&0.938&0.970&\textbf{0.973}&0.966\\
\bottomrule
\end{tabular}}
\label{tab5:depth}
%\vspace{-4pt}
\end{table} 

==> tables/table7.tex <==
\begin{table*}
\begin{floatrow}

\begin{minipage}[!t]{0.39\linewidth}
\vspace{0pt}
\centering
\ttabbox{\caption{Performance comparison for mask detection on three benchmark datasets.
\vspace{-4pt}}
\label{tab1:mask}}
{
\resizebox{0.9\linewidth}{!}{
\begin{tabular}{c |l| c c c c c c}
\toprule
%\multirow{2}*{Metric}&\multirow{2}*{Method}
\multicolumn{2}{c|}{Dataset}&\multicolumn{2}{c}{FFHQ~\cite{karras2019style}} &\multicolumn{2}{c}{ImageNet~\cite{deng2009imagenet}}&\multicolumn{2}{c}{Places~\cite{zhou2017places}} \\
% \cmidrule(lr){3-5} 
% \cmidrule(lr){6-8}
% \cmidrule(lr){9-11}
\cmidrule(lr){1-2}
\cmidrule(lr){3-4} 
\cmidrule(lr){5-6}
\cmidrule(lr){7-8}
%~&&small&large&small&large&small&large\\
\multicolumn{2}{c|}{Mask ratio (\%)}&0-30&30-60&0-30&30-60&0-30&30-60\\
\midrule
\multirow{2}*{Acc~$\uparrow$}&VCNet&0.948&0.943&0.972&0.978&0.974&0.976 \\
~&Ours&\textbf{0.978}&\textbf{0.976}&\textbf{0.982}&\textbf{0.983}&\textbf{0.984}&\textbf{0.985} \\
\midrule
\multirow{2}*{F1~$\uparrow$}&VCNet&0.967&0.948&0.982&0.980&0.984&0.978\\
~&Ours&\textbf{0.986}&\textbf{0.978}&\textbf{0.989}&\textbf{0.985}&\textbf{0.991}&\textbf{0.987} \\
\midrule
\multirow{2}*{BCE~$\downarrow$}&VCNet&0.126&0.137&\textbf{0.073}&\textbf{0.055}&\textbf{0.064}&\textbf{0.060} \\
~&Ours&\textbf{0.090}&\textbf{0.095}&0.083&0.075&0.068&0.064 \\
\midrule
\multirow{2}*{IoU~$\uparrow$}&VCNet&0.931&0.900&0.966&0.962&0.969&0.959 \\
~&Ours&\textbf{0.975}&\textbf{0.959}&\textbf{0.978}&\textbf{0.965}&\textbf{0.982}&\textbf{0.974} \\
\bottomrule
\end{tabular}}
}
\end{minipage}
%\hspace{0.5mm}

\begin{minipage}[!t]{0.575\linewidth}
\vspace{0pt}
\centering
\ttabbox{\caption{Performance comparison for blind image inpainting in terms of four evaluation metrics on three benchmark datasets.
\vspace{-4pt}}
\label{tab2:blind}}
{
%\resizebox{0.975\linewidth}{!}{
\resizebox{0.9\linewidth}{!}{
 \begin{tabular}{c| l| c c c c| c c c c| c c c c}
\toprule
\multicolumn{2}{c|}{Dataset}&\multicolumn{4}{c|}{FFHQ~\cite{karras2019style}} &\multicolumn{4}{c|}{ImageNet~\cite{deng2009imagenet}}&\multicolumn{4}{c}{Places~\cite{zhou2017places}} \\
\cmidrule(lr){1-2} 
\cmidrule(lr){3-6} 
\cmidrule(lr){7-10}
\cmidrule(lr){11-14}
\multicolumn{2}{c|}{Mask ratio (\%)}&0-20 & 20-40 & 40-60 & 0-60 &0-20 & 20-40 & 40-60 & 0-60 &0-20 & 20-40 & 40-60 & 0-60 \\
\midrule
\multirow{3}*{PSNR~$\uparrow$}&MPRNet&33.93&26.75&22.06&27.58&33.76&26.26&21.50&27.17&33.37&25.59&21.08&26.68 \\
~&VCNet&29.86&24.51&20.51&24.96&29.13&23.39&19.42&23.98&29.66&23.19&19.18&24.01 \\
~&Ours&\textbf{34.79}&\textbf{27.98}&\textbf{23.54}&\textbf{28.77}&\textbf{33.91}&\textbf{26.40}&\textbf{21.80}&\textbf{27.37}&\textbf{34.11}&\textbf{26.20}&\textbf{21.66}&\textbf{27.32} \\
\midrule
\multirow{3}*{SSIM~$\uparrow$}&MPRNet&0.968&0.898&0.799&0.888&0.965&0.882&0.762&0.870&0.965&0.876&0.748&0.863 \\
~&VCNet&0.933&0.849&0.736&0.839&0.924&0.818&0.678&0.807&0.942&0.833&0.688&0.821 \\
~&Ours&\textbf{0.971}&\textbf{0.910}&\textbf{0.824}&\textbf{0.901}&\textbf{0.966}&\textbf{0.884}&\textbf{0.767}&\textbf{0.872}&\textbf{0.969}&\textbf{0.887}&\textbf{0.746}&\textbf{0.873} \\
\midrule
\multirow{3}*{FID~$\downarrow$}&MPRNet&3.37&12.20&29.74&15.11&3.71&17.80&53.38&24.96&4.15&17.61&44.73&22.16 \\
~&VCNet&6.80&14.17&28.90&16.63&5.69&21.48&59.11&28.76&5.93&18.62&40.21&21.59 \\
~&Ours&\textbf{2.37}&\textbf{7.28}&\textbf{15.48}&\textbf{8.38}&\textbf{2.69}&\textbf{12.35}&\textbf{41.37}&\textbf{18.80}&\textbf{2.88}&\textbf{11.10}&\textbf{31.33}&\textbf{15.10} \\
\midrule
\multirow{3}*{LPIPS~$\downarrow$}&MPRNet&0.027&0.096&0.212&0.112&0.033&0.123&0.269&0.141&0.033&0.131&0.283&0.149 \\
~&VCNet&0.044&0.103&0.188&0.112&0.045&0.128&0.246&0.140&0.046&0.138&0.261&0.148 \\
~&Ours&\textbf{0.019}&\textbf{0.065}&\textbf{0.139}&\textbf{0.075}&\textbf{0.025}&\textbf{0.098}&\textbf{0.226}&\textbf{0.116}&\textbf{0.024}&\textbf{0.095}&\textbf{0.221}&\textbf{0.113} \\
\bottomrule
\end{tabular}}
}
\end{minipage}

\end{floatrow}
\vspace{-8pt}
\end{table*}


==> tables/table8.tex <==
\begin{table*}
\begin{floatrow}

\capbtabbox{
\resizebox{0.85\linewidth}{!}{
\begin{tabular}{c |l| c c c c c c}
\toprule
%\multirow{2}*{Metric}&\multirow{2}*{Method}
\multicolumn{2}{c|}{Dataset}&\multicolumn{2}{c}{FFHQ~\cite{karras2019style}} &\multicolumn{2}{c}{ImageNet~\cite{deng2009imagenet}}&\multicolumn{2}{c}{Places~\cite{zhou2017places}} \\
% \cmidrule(lr){3-5} 
% \cmidrule(lr){6-8}
% \cmidrule(lr){9-11}
\cmidrule(lr){1-2}
\cmidrule(lr){3-4} 
\cmidrule(lr){5-6}
\cmidrule(lr){7-8}
%~&&small&large&small&large&small&large\\
\multicolumn{2}{c|}{Mask ratio (\%)}&0-30&30-60&0-30&30-60&0-30&30-60\\
\midrule
\multirow{2}*{Acc~$\uparrow$}&VCNet&0.948&0.943&0.972&0.978&0.974&0.976 \\
~&Ours&\textbf{0.978}&\textbf{0.976}&\textbf{0.982}&\textbf{0.983}&\textbf{0.984}&\textbf{0.985} \\
\midrule
\multirow{2}*{F1~$\uparrow$}&VCNet&0.967&0.948&0.982&0.980&0.984&0.978\\
~&Ours&\textbf{0.986}&\textbf{0.978}&\textbf{0.989}&\textbf{0.985}&\textbf{0.991}&\textbf{0.987} \\
\midrule
\multirow{2}*{BCE~$\downarrow$}&VCNet&0.126&0.137&\textbf{0.073}&\textbf{0.055}&\textbf{0.064}&\textbf{0.060} \\
~&Ours&\textbf{0.090}&\textbf{0.095}&0.083&0.075&0.068&0.064 \\
\midrule
\multirow{2}*{IoU~$\uparrow$}&VCNet&0.931&0.900&0.966&0.962&0.969&0.959 \\
~&Ours&\textbf{0.975}&\textbf{0.959}&\textbf{0.978}&\textbf{0.965}&\textbf{0.982}&\textbf{0.974} \\
\bottomrule
\end{tabular}}
}
{
 \captionsetup{width=.4\textwidth}
 \caption{Performance comparison for mask detection on three benchmark datasets for blind image inpainting.}
 \label{tab1:mask}
}

%\hspace{3mm}
\capbtabbox{
 \resizebox{1.05\linewidth}{!}{
 \begin{tabular}{c| l| c c c c| c c c c| c c c c}
\toprule
\multicolumn{2}{c|}{Dataset}&\multicolumn{4}{c|}{FFHQ~\cite{karras2019style}} &\multicolumn{4}{c|}{ImageNet~\cite{deng2009imagenet}}&\multicolumn{4}{c}{Places~\cite{zhou2017places}} \\
\cmidrule(lr){1-2} 
\cmidrule(lr){3-6} 
\cmidrule(lr){7-10}
\cmidrule(lr){11-14}
\multicolumn{2}{c|}{Mask ratio (\%)}&0-20 & 20-40 & 40-60 & 0-60 &0-20 & 20-40 & 40-60 & 0-60 &0-20 & 20-40 & 40-60 & 0-60 \\
\midrule
\multirow{2}*{PSNR~$\uparrow$}&VCNet&29.86&24.51&20.51&24.96&29.13&23.39&19.42&23.98&29.66&23.19&19.18&24.01 \\
~&Ours&\textbf{34.79}&\textbf{27.98}&\textbf{23.54}&\textbf{28.77}&\textbf{33.91}&\textbf{26.40}&\textbf{21.80}&\textbf{27.37}&\textbf{34.11}&\textbf{26.20}&\textbf{21.66}&\textbf{27.32} \\
\midrule
\multirow{2}*{SSIM~$\uparrow$}&VCNet&0.933&0.849&0.736&0.839&0.924&0.818&0.678&0.807&0.942&0.833&0.688&0.821 \\
~&Ours&\textbf{0.971}&\textbf{0.910}&\textbf{0.824}&\textbf{0.901}&\textbf{0.966}&\textbf{0.884}&\textbf{0.767}&\textbf{0.872}&\textbf{0.969}&\textbf{0.887}&\textbf{0.746}&\textbf{0.873} \\
\midrule
\multirow{2}*{FID~$\downarrow$}&VCNet&6.80&14.17&28.90&16.63&5.69&21.48&59.11&28.76&5.93&18.62&40.21&21.59 \\
~&Ours&\textbf{2.37}&\textbf{7.28}&\textbf{15.48}&\textbf{8.38}&\textbf{2.69}&\textbf{12.35}&\textbf{41.37}&\textbf{18.80}&\textbf{2.88}&\textbf{11.10}&\textbf{31.33}&\textbf{15.10} \\
\midrule
\multirow{2}*{LPIPS~$\downarrow$}&VCNet&0.044&0.103&0.188&0.112&0.045&0.128&0.246&0.140&0.046&0.138&0.261&0.148 \\
~&Ours&\textbf{0.019}&\textbf{0.065}&\textbf{0.139}&\textbf{0.075}&\textbf{0.025}&\textbf{0.098}&\textbf{0.226}&\textbf{0.116}&\textbf{0.024}&\textbf{0.095}&\textbf{0.221}&\textbf{0.113} \\
\bottomrule
\end{tabular}}
}{

 \captionsetup{width=0.6\textwidth}
  \caption{Performance comparison for blind image inpainting in terms of four evaluation metrics on three benchmark datasets.}
 \label{tab2:blind}
}

\end{floatrow}
\vspace{-4pt}
\end{table*}


==> tables/table_combine.tex <==
\begin{table*}
\begin{floatrow}
\begin{minipage}[!t]{0.575\linewidth}
\vspace{0pt}
\centering
\ttabbox{\caption{Performance comparison for blind image inpainting in terms of four evaluation metrics on three benchmark datasets.
\vspace{-4pt}}
\label{tab2:blind}}
{
\resizebox{1\linewidth}{!}{
 \begin{tabular}{c| l| c c c c| c c c c| c c c c}
\toprule
\multicolumn{2}{c|}{Dataset}&\multicolumn{4}{c|}{FFHQ~\cite{karras2019style}} &\multicolumn{4}{c|}{ImageNet~\cite{deng2009imagenet}}&\multicolumn{4}{c}{Places~\cite{zhou2017places}} \\
\cmidrule(lr){1-2} 
\cmidrule(lr){3-6} 
\cmidrule(lr){7-10}
\cmidrule(lr){11-14}
\multicolumn{2}{c|}{Mask ratio (\%)}&0-20 & 20-40 & 40-60 & 0-60 &0-20 & 20-40 & 40-60 & 0-60 &0-20 & 20-40 & 40-60 & 0-60 \\
\midrule
\multirow{3}*{PSNR~$\uparrow$}&MPRNet&33.93&26.75&22.06&27.58&33.76&26.26&21.50&27.17&33.37&25.59&21.08&26.68 \\
~&VCNet&29.86&24.51&20.51&24.96&29.13&23.39&19.42&23.98&29.66&23.19&19.18&24.01 \\
~&Ours&\textbf{34.79}&\textbf{27.98}&\textbf{23.54}&\textbf{28.77}&\textbf{33.91}&\textbf{26.40}&\textbf{21.80}&\textbf{27.37}&\textbf{34.11}&\textbf{26.20}&\textbf{21.66}&\textbf{27.32} \\
\midrule
\multirow{3}*{SSIM~$\uparrow$}&MPRNet&0.968&0.898&0.799&0.888&0.965&0.882&0.762&0.870&0.965&0.876&0.748&0.863 \\
~&VCNet&0.933&0.849&0.736&0.839&0.924&0.818&0.678&0.807&0.942&0.833&0.688&0.821 \\
~&Ours&\textbf{0.971}&\textbf{0.910}&\textbf{0.824}&\textbf{0.901}&\textbf{0.966}&\textbf{0.884}&\textbf{0.767}&\textbf{0.872}&\textbf{0.969}&\textbf{0.887}&\textbf{0.746}&\textbf{0.873} \\
\midrule
\multirow{3}*{FID~$\downarrow$}&MPRNet&3.37&12.20&29.74&15.11&3.71&17.80&53.38&24.96&4.15&17.61&44.73&22.16 \\
~&VCNet&6.80&14.17&28.90&16.63&5.69&21.48&59.11&28.76&5.93&18.62&40.21&21.59 \\
~&Ours&\textbf{2.37}&\textbf{7.28}&\textbf{15.48}&\textbf{8.38}&\textbf{2.69}&\textbf{12.35}&\textbf{41.37}&\textbf{18.80}&\textbf{2.88}&\textbf{11.10}&\textbf{31.33}&\textbf{15.10} \\
\midrule
\multirow{3}*{LPIPS~$\downarrow$}&MPRNet&0.027&0.096&0.212&0.112&0.033&0.123&0.269&0.141&0.033&0.131&0.283&0.149 \\
~&VCNet&0.044&0.103&0.188&0.112&0.045&0.128&0.246&0.140&0.046&0.138&0.261&0.148 \\
~&Ours&\textbf{0.019}&\textbf{0.065}&\textbf{0.139}&\textbf{0.075}&\textbf{0.025}&\textbf{0.098}&\textbf{0.226}&\textbf{0.116}&\textbf{0.024}&\textbf{0.095}&\textbf{0.221}&\textbf{0.113} \\
\bottomrule
\end{tabular}}}
\end{minipage}

\begin{minipage}[!t]{0.39\linewidth}
\vspace{0pt}
\centering
\ttabbox{\caption{Performance evaluation on watermark removal.
\vspace{-4pt}}
\label{tab4:watermark}}
{
\resizebox{1\linewidth}{!}{
\begin{tabular}{l | ccc}
\toprule
Metrics& PSNR$\uparrow$ & SSIM$\uparrow$ & FID$\downarrow$\\
\midrule
SIRF~\cite{zhang2018single}    &34.63&0.978&0.071 \\ 
BS$^2$AM~\cite{cun2020improving}&34.88&0.979&0.028 \\ 
DHAN~\cite{cun2020towards}    &37.67&0.986&0.062 \\ 
BVMR~\cite{hertz2019blind}    &38.28&0.985&0.018 \\ 
Split then Refine~\cite{cun2021split} &41.27&0.991&0.011 \\ 
VCNet~\cite{wang2020vcnet}   &32.66&0.963&0.032 \\ 
Ours       &\textbf{41.88}&\textbf{0.992}&\textbf{0.007} \\ 
\bottomrule
\end{tabular}
 }}
\end{minipage}
\end{floatrow}
\vspace{-8pt}
\end{table*}

